Question Personalization in an Intelligent Tutoring System

This paper investigates personalization in the field of intelligent tutoring systems (ITS). We hypothesize that personalization in the way questions are asked improves student learning outcomes. Previous work on dialogue-based ITS personalization has yet to address question phrasing. We show that generating versions of the questions suitable for students at different levels of subject proficiency improves student learning gains, using variants written by a domain expert and an experimental A/B test. This insight demonstrates that the linguistic realization of questions in an ITS affects the learning outcomes for students.

==> sections/results_outdated.tex <==
% TO DO: recalculate the statistical significance between the table entries & include alpha value --> currently none have a p-value <= 0.05... hopefully with more data

In order to test our claims we ran an AB test with three groups on the \texttt{AI Tutor} platform. Each time a user in the \textit{selected variant} group encountered an exercise in our experiment, they received a question variant matched to their level according to the model explained in section \ref{methods}. The \textit{random variant} group received a random variant each time they encountered an exercise in our experiment. This group was included to verify that the success of the \textit{selected variant} group is due to the variants being matched to their level, not due other differences between the variants and the original. The final group in the AB test is a \textit{control} group, who received the original exercises from the \texttt{AI Tutor}. Note that users who skipped at least 25\% of the exercises, or those who completed less than 10 exercises were excluded from the results reported below.

Table \ref{tab2} contains the results of the three experimental groups on three different metrics. First, the \textit{eventual success rate} metric represents if a student succeeded on an exercise, regardless of the number of attempts they needed. The \textit{selected variant} group performed the best, with an over 10\% increase in their \textit{eventual success rate}. The \textit{random variant} and \textit{control} groups performed similarly, indicating that not matching question variant levels to students produces similar results to not having question variants at all. 

Succeeding on exercises does not equate to learning. The best learning occurs when the student is challenged but can still obtain the right answer with hints, otherwise known as the zone of proximal development \cite{cazden_1979}. Therefore, we want to maximize the \textit{average number of failed attempts per exercise} along with the \textit{eventual success rate}. The \textit{random variant} group has the highest score in this metric, which follows as beginner level users in this category are likely to struggle on advanced level variants. The \textit{selected variant} group still performs well here, with statistically significant increase in the metric over the control group.

The \textit{average skip rate} metric can indicate the engagement of the students within the different experiment groups. All three groups have quite low skip rates, and are close to one another. The \textit{selected variant} group does have the lowest rate, in line with our hypothesis.

\vspace*{-1\baselineskip}
\begin{table} \begin{center}
    \caption{AB test group results on various metrics.} \label{tab2}
    \begin{tabular}{| c | c | c | c | c |}
    \hline
    Experiment Group & \begin{tabular}{@{}c@{}}Eventual Success \\ Rate \end{tabular} & \begin{tabular}{@{}c@{}} Failed Attempts \\ per Exercise \end{tabular} & Skip Rate & n\\
    \hline
    Selected Variant & 0.871 $\pm$ 0.040 &  0.419 $\pm$ 0.086 & 0.000 $\pm$ 0.000 & 31\\
    Random Variant & 0.725 $\pm$ 0.062 & 0.500 $\pm$ 0.078 & 0.075 $\pm$ 0.021 & 40\\
    Control & 0.739 $\pm$ 0.056 & 0.326 $\pm$ 0.064 & 0.022 $\pm$ 0.006 & 46\\
    \hline
    \end{tabular}
\end{center} \end{table} \vspace*{-2\baselineskip}

Finally, we can look at the results from both variant groups through a different lens to further color our understanding. Throughout the course of the experiment there were 228 attempts on variant exercises by users. Of those, 123 variants were assigned to users matched to the level of the variant, called the \textit{expected variant} group. The other 105 variants were assigned to users who did not match their level, called the \textit{non expected variant} group. We will compare their \textit{attempt success rate}, which represents the success rate across all attempts, as opposed to all exercises encountered. The \textit{expected variant} group had an \textit{attempt success rate} of $0.650 \pm 0.084$, and the \textit{non expected variant} group's was $0.448 \pm 0.095$. The difference between the two is statistically significant with a p-value of $0.002$ and an $\alpha = 0.05$.

Looking at all of the metrics presented above, we can see a clear improvement in the learning gains of students in the \textit{selected variant} group over the other two groups. These results support our hypothesis that providing question variants suited to student's level will improve their learning gains. 
